The Density of States in the Two-Dimensional Electron Gas and Quantum Dots (Ph.D. thesis, Cornell University, January 1991)

This thesis describes capacitance and tunneling experiments performed on two-dimensional electron gas (2DEG) and quantum dot systems. It develops a system of equations that allow determination, by means of capacitance measurements, of the electronic density of states, the electron density, and the chemical potential in a 2DEG. The thesis describes the use of these techniques in the observation of a magnetic field induced energy gap to tunneling in the 2DEG and the single electron addition spectrum in arrays of quantum dots.

==> bbibitems.tex <==
\bibitem{DICK-bridge}{R.E. Cavicchi and R.H. Silsbee, Rev.\ Sci.\
Instrum.\ {\bf 59}, 176, (1988)}
\bibitem{YOPRL}{R.C. Ashoori, J.A. Lebens, N.P. Bigelow, and R.H.
Silsbee, \PRL{64}{6}{1990}}
\bibitem{CHAP6}{{\it See Chapter 6}}
\bibitem{CHAP4}{{\it See Chapter 4}}
%
\bibitem{HORO&HILL}{Paul Horowitz and Winfield Hill, {\it The Art of
Electronics} (Cambridge University Press, 1989)}


==> figmac.tex <==
% figmac.tex 1-30-87  ** requires REFMAC.TEX 10.8.86 or newer **
%
% This file contains a set of macros to be input after
% REFMAC.TEX and EQNMAC.TEX that enable keyword substitution for figure
% numbers.  When a new figure is written, one types
%       \newfig{key}
% and the next available figure number will be printed.
% To print the figure number(s) associated with a particular
% key(s) after the initial entry, just type
%       \fignum{key1,key2,key3}           (with no spaces)
% and the figure numbers will be printed in sequential order,
% separated by commas, and with any sequence of 3 or more hyphenated
% (i.e. 1,2,3 -> 1-3).
%

% in REFMAC.TEX, namely \add#1\to#2 and \citedef#1#2,
% and EQNMAC.TEX, namely \createlist#1 and \concatlist#1.
%
%\tracingmacros=1
%\tracingmacros=2
%\tracingonline=1
%
\immediate\write16{** FIGMAC.TEX...figure numbering macros...LJW1.30.87 **}
%
\def\figkeys{}    % the key list macro
\newcount\figcnt  % the current figure number
\figcnt=0
\def\newfig#1{\global\advance\figcnt by 1\add{#1}\to{\figkeys}\number\figcnt}
%
% The next macro, \fignum#1, prints the figure numbers associated
% with particular keys the same way that \refnumber prints the
% reference numbers.  First it puts the keys into a list macro with
% \createlist#1, keeping track of how many are noted with \listcnt,
% then \findfignum#1 uses the \citedef#1#2 macro to
% search the \figkeys list for noted figure keys and print them in
% the appropriate format.
%
\def\fignum#1{\createlist{#1}\findfignum{\listed}}
\def\findfignum#1{\refnum=0%
                  \seqnum=0%
                  \citenum=\listcnt%
                  \def\\##1{\citedef{#1}{##1}}%
                  \figkeys%
                  \def\\##1{}}
%
% That's all folks!


==> manmac.tex <==
% Macros for The TeXbook

\catcode`@=11 % borrow the private macros of PLAIN (with care)

\font\tentex=cmtex10

\font\inchhigh=cminch
\font\titlefont=cmssdc10 at 40pt

\font\ninerm=cmr9
\font\eightrm=cmr8
\font\sixrm=cmr6

\font\ninei=cmmi9
\font\eighti=cmmi8
\font\sixi=cmmi6
\skewchar\ninei='177 \skewchar\eighti='177 \skewchar\sixi='177

\font\ninesy=cmsy9
\font\eightsy=cmsy8
\font\sixsy=cmsy6
\skewchar\ninesy='60 \skewchar\eightsy='60 \skewchar\sixsy='60

\font\eightss=cmssq8

\font\eightssi=cmssqi8

\font\ninebf=cmbx9
\font\eightbf=cmbx8
\font\sixbf=cmbx6

\font\ninett=cmtt9
\font\eighttt=cmtt8

\hyphenchar\tentt=-1 % inhibit hyphenation in typewriter type
\hyphenchar\ninett=-1
\hyphenchar\eighttt=-1

\font\ninesl=cmsl9
\font\eightsl=cmsl8

\font\nineit=cmti9
\font\eightit=cmti8

\font\tenu=cmu10 % unslanted text italic
\font\magnifiedfiverm=cmr5 at 10pt
\font\manual=manfnt % font used for the METAFONT logo, etc.
\font\cmman=cmman % font used for miscellaneous Computer Modern variations

\newskip\ttglue
\def\tenpoint{\def\rm{\fam0\tenrm}%
  \textfont0=\tenrm \scriptfont0=\sevenrm \scriptscriptfont0=\fiverm
  \textfont1=\teni \scriptfont1=\seveni \scriptscriptfont1=\fivei
  \textfont2=\tensy \scriptfont2=\sevensy \scriptscriptfont2=\fivesy
  \textfont3=\tenex \scriptfont3=\tenex \scriptscriptfont3=\tenex
  \def\it{\fam\itfam\tenit}%
  \textfont\itfam=\tenit
  \def\sl{\fam\slfam\tensl}%
  \textfont\slfam=\tensl
  \def\bf{\fam\bffam\tenbf}%
  \textfont\bffam=\tenbf \scriptfont\bffam=\sevenbf
   \scriptscriptfont\bffam=\fivebf
  \def\tt{\fam\ttfam\tentt}%
  \textfont\ttfam=\tentt
  \tt \ttglue=.5em plus.25em minus.15em
  \normalbaselineskip=12pt
  \def\MF{{\manual META}\-{\manual FONT}}%
  \let\sc=\eightrm
  \let\big=\tenbig
  \setbox\strutbox=\hbox{\vrule height8.5pt depth3.5pt width\z@}%
  \normalbaselines\rm}

\def\ninepoint{\def\rm{\fam0\ninerm}%
  \textfont0=\ninerm \scriptfont0=\sixrm \scriptscriptfont0=\fiverm
  \textfont1=\ninei \scriptfont1=\sixi \scriptscriptfont1=\fivei
  \textfont2=\ninesy \scriptfont2=\sixsy \scriptscriptfont2=\fivesy
  \textfont3=\tenex \scriptfont3=\tenex \scriptscriptfont3=\tenex
  \def\it{\fam\itfam\nineit}%
  \textfont\itfam=\nineit
  \def\sl{\fam\slfam\ninesl}%
  \textfont\slfam=\ninesl
  \def\bf{\fam\bffam\ninebf}%
  \textfont\bffam=\ninebf \scriptfont\bffam=\sixbf
   \scriptscriptfont\bffam=\fivebf
  \def\tt{\fam\ttfam\ninett}%
  \textfont\ttfam=\ninett
  \tt \ttglue=.5em plus.25em minus.15em
  \normalbaselineskip=11pt
  \def\MF{{\manual hijk}\-{\manual lmnj}}%
  \let\sc=\sevenrm
  \let\big=\ninebig
  \setbox\strutbox=\hbox{\vrule height8pt depth3pt width\z@}%
  \normalbaselines\rm}

\def\eightpoint{\def\rm{\fam0\eightrm}%
  \textfont0=\eightrm \scriptfont0=\sixrm \scriptscriptfont0=\fiverm
  \textfont1=\eighti \scriptfont1=\sixi \scriptscriptfont1=\fivei
  \textfont2=\eightsy \scriptfont2=\sixsy \scriptscriptfont2=\fivesy
  \textfont3=\tenex \scriptfont3=\tenex \scriptscriptfont3=\tenex
  \def\it{\fam\itfam\eightit}%
  \textfont\itfam=\eightit
  \def\sl{\fam\slfam\eightsl}%
  \textfont\slfam=\eightsl
  \def\bf{\fam\bffam\eightbf}%
  \textfont\bffam=\eightbf \scriptfont\bffam=\sixbf
   \scriptscriptfont\bffam=\fivebf
  \def\tt{\fam\ttfam\eighttt}%
  \textfont\ttfam=\eighttt
  \tt \ttglue=.5em plus.25em minus.15em
  \normalbaselineskip=9pt
  \def\MF{{\manual opqr}\-{\manual stuq}}%
  \let\sc=\sixrm
  \let\big=\eightbig
  \setbox\strutbox=\hbox{\vrule height7pt depth2pt width\z@}%
  \normalbaselines\rm}

\def\tenmath{\tenpoint\fam-1 } % use after $ in ninepoint sections
\def\tenbig#1{{\hbox{$\left#1\vbox to8.5pt{}\right.\n@space$}}}
\def\ninebig#1{{\hbox{$\textfont0=\tenrm\textfont2=\tensy
  \left#1\vbox to7.25pt{}\right.\n@space$}}}
\def\eightbig#1{{\hbox{$\textfont0=\ninerm\textfont2=\ninesy
  \left#1\vbox to6.5pt{}\right.\n@space$}}}

% Page layout
\newdimen\pagewidth \newdimen\pageheight \newdimen\ruleht
\hsize=29pc  \vsize=44pc  \maxdepth=2.2pt  \parindent=3pc
\pagewidth=\hsize \pageheight=\vsize \ruleht=.5pt
\abovedisplayskip=6pt plus 3pt minus 1pt
\belowdisplayskip=6pt plus 3pt minus 1pt
\abovedisplayshortskip=0pt plus 3pt
\belowdisplayshortskip=4pt plus 3pt

%\newinsert\footins
\def\footnote#1{\edef\@sf{\spacefactor\the\spacefactor}#1\@sf
      \insert\footins\bgroup\eightpoint
      \interlinepenalty100 \let\par=\endgraf
        \leftskip=\z@skip \rightskip=\z@skip
        \splittopskip=10pt plus 1pt minus 1pt \floatingpenalty=20000
        \smallskip\item{#1}\bgroup\strut\aftergroup\@foot\let\next}
\skip\footins=12pt plus 2pt minus 4pt % space added when footnote is present
%\count\footins=1000 % footnote magnification factor (1 to 1)
\dimen\footins=30pc % maximum footnotes per page

\newinsert\margin
\dimen\margin=\maxdimen
%\count\margin=0 \skip\margin=0pt % marginal inserts take up no space

\newif\iftitle
\def\titlepage{\global\titletrue} % for pages without headlines
\def\rhead{} % \rhead contains the running headline

\def\leftheadline{\hbox to \pagewidth{%
    \vbox to 10pt{}% strut to position the baseline
    \llap{\tenbf\folio\kern1pc}% folio to left of text
    \tenit\rhead\hfil% running head flush left
    }}
\def\rightheadline{\hbox to \pagewidth{%
    \vbox to 10pt{}% strut to position the baseline
    \hfil\tenit\rhead\/% running head flush right
    \rlap{\kern1pc\tenbf\folio}% folio to right of text
    }}

\def\onepageout#1{\shipout\vbox{ % here we define one page of output
    \offinterlineskip % butt the boxes together
    \vbox to 3pc{ % this part goes on top of the 44pc pages
      \iftitle % the next is used for title pages
        \global\titlefalse % reset the titlepage switch
        \setcornerrules % for camera alignment
      \else\ifodd\pageno \rightheadline\else\leftheadline\fi\fi
      \vfill} % this completes the \vbox to 3pc
    \vbox to \pageheight{
      \ifvoid\margin\else % marginal info is present
        \rlap{\kern31pc\vbox to\z@{\kern4pt\box\margin \vss}}\fi
      #1 % now insert the main information
      \ifvoid\footins\else % footnote info is present
        \vskip\skip\footins \kern-3pt
        \hrule height\ruleht width\pagewidth \kern-\ruleht \kern3pt
        \unvbox\footins\fi
      \boxmaxdepth=\maxdepth
      } % this completes the \vbox to \pageheight
    }
  \advancepageno}

\def\setcornerrules{\hbox to \pagewidth{\vrule width 1pc height\ruleht
    \hfil \vrule width 1pc}
  \hbox to \pagewidth{\llap{\sevenrm(page \folio)\kern1pc}%
    \vrule height1pc width\ruleht depth\z@
    \hfil \vrule width\ruleht depth\z@}}

\output{\onepageout{\unvbox255}}

\newbox\partialpage
\def\begindoublecolumns{\begingroup
  \output={\global\setbox\partialpage=\vbox{\unvbox255\bigskip}}\eject
  \output={\doublecolumnout} \hsize=14pc \vsize=89pc}
\def\enddoublecolumns{\output={\balancecolumns}\eject
  \endgroup \pagegoal=\vsize}

\def\doublecolumnout{\splittopskip=\topskip \splitmaxdepth=\maxdepth
  \dimen@=44pc \advance\dimen@ by-\ht\partialpage
  \setbox0=\vsplit255 to\dimen@ \setbox2=\vsplit255 to\dimen@
  \onepageout\pagesofar
  \unvbox255 \penalty\outputpenalty}
\def\pagesofar{\unvbox\partialpage
  \wd0=\hsize \wd2=\hsize \hbox to\pagewidth{\box0\hfil\box2}}
\def\balancecolumns{\setbox0=\vbox{\unvbox255} \dimen@=\ht0
  \advance\dimen@ by\topskip \advance\dimen@ by-\baselineskip
  \divide\dimen@ by2 \splittopskip=\topskip
  {\vbadness=10000 \loop \global\setbox3=\copy0
    \global\setbox1=\vsplit3 to\dimen@
    \ifdim\ht3>\dimen@ \global\advance\dimen@ by1pt \repeat}
  \setbox0=\vbox to\dimen@{\unvbox1}
  \setbox2=\vbox to\dimen@{\unvbox3}
  \pagesofar}

% To produce only a subset of pages, put the page numbers on separate
% lines in a file called pages.tex
\let\Shipout=\shipout
\newread\pages \newcount\nextpage \openin\pages=pages
\def\getnextpage{\ifeof\pages\else
 {\endlinechar=-1\read\pages to\next
  \ifx\next\empty % in this case we should have eof now
  \else\global\nextpage=\next\fi}\fi}
\ifeof\pages\else\message{OK, I'll ship only the requested pages!}
 \getnextpage\fi
\def\shipout{\ifeof\pages\let\next=\Shipout
 \else\ifnum\pageno=\nextpage\getnextpage\let\next=\Shipout
  \else\let\next=\Tosspage\fi\fi \next}
\newbox\garbage \def\Tosspage{\deadcycles=0\setbox\garbage=}

% Chapter formatting
% The preface and table of contents are formatted in place, not here

\newcount\exno % for the number of exercises in the current chapter
\newcount\subsecno % for the number of subsections in the current chapter

\def\beginchapter#1 #2#3. #4\par{\global\exno=0
  \subsecno=0
  \def\chapno{#2#3}
  \ifodd\pageno
    \errmessage{You had too much text on that last page; I'm backing up}
    \advance\pageno by-1 \fi
  \titlepage
  \def\\{ } % \\'s in the title will be treated as spaces
  \message{#1 #2#3:} % show the chapter title on the terminal
  \def\MF{{\manual 89:;<=>:}} % slant the logo
  \xdef\rhead{#1 #2#3: #4\unskip}
  {\def\TeX{T\kern-.2em\lower.5ex\hbox{E}\kern-.06em X}
    \def\MF{{\vbox to30pt{}\manual ()*+,-.*}}
    \def\\{#3}
    \ifx\empty\\ \rightline{\inchhigh #2\kern-.04em}
    \else\rightline{\inchhigh #2\kern-.06em#3\kern-.04em}\fi
    \vskip 1.75pc
    \baselineskip 36pt \lineskiplimit \titlelsl \lineskip 12pt
    \let\\=\cr % now the \\'s are line dividers
    \halign{\line{\titlefont\hfil##}\\#4\unskip\\}
    \vfill\eject} % output the chapter title page
  \tenpoint
  \noindent\ignorespaces} % the first paragraph of a chapter is not indented
\newdimen\titlelsl \titlelsl=1pt

\outer\def\endchapter{\ifodd\pageno \else\vfill\eject\null\fi
  \begingroup\bigskip\vfill % beginning of the quotes
  \def\eject{\endgroup\eject}
  \def\par{\ifhmode\/\endgraf\fi}\obeylines
  \def\TeX{T\kern-.2em\lower.5ex\hbox{E}\kern-.000em X}
  \def\MF{{\manual opqr}\-{\manual stuq}}
  \eightpoint \let\tt=\ninett
  \baselineskip 10pt
  \parfillskip \z@
  \interlinepenalty 10000
  \leftskip \z@ plus 40pc minus \parindent
  \let\rm=\eightss \let\sl=\eightssi
  \everypar{\sl}}
\def\author#1(#2){\smallskip\noindent\rm--- #1\unskip\enspace(#2)}

\def\dbend{{\manual\char127}} % dangerous bend sign
\def\d@nger{\medbreak\begingroup\clubpenalty=10000
  \def\par{\endgraf\endgroup\medbreak} \noindent\hang\hangafter=-2
  \hbox to0pt{\hskip-\hangindent\dbend\hfill}\ninepoint}
\outer\def\danger{\d@nger}
\def\dd@nger{\medbreak\begingroup\clubpenalty=10000
  \def\par{\endgraf\endgroup\medbreak} \noindent\hang\hangafter=-2
  \hbox to0pt{\hskip-\hangindent\dbend\kern1pt\dbend\hfill}\ninepoint}
\outer\def\ddanger{\dd@nger}
\def\enddanger{\endgraf\endgroup} % omits the \medbreak

\outer\def\subsection#1. {\medbreak\advance\subsecno by 1
  \noindent{\it \the\subsecno.\enspace#1.\enspace}}
\def\ansno#1.#2:{\medbreak\noindent
  \hbox to\parindent{\bf\hss#1.#2.\enspace}\ignorespaces}

% Composition macros
\hyphenation{man-u-script man-u-scripts ap-pen-dix xscaled}

\def\AmSTeX{$\cal A\kern-.1667em\lower.5ex\hbox{$\cal M$}\kern-.075em
  S$-\TeX}
\def\bull{\vrule height .9ex width .8ex depth -.1ex } % square bullet
\def\SS{{\it SS}} % scriptscript style
\def\|{\leavevmode\hbox{\tt\char`\|}} % vertical line
\def\dn{\leavevmode\hbox{\tt\char'14}} % downward arrow
\def\up{\leavevmode\hbox{\tt\char'13}} % upward arrow
\def\]{\leavevmode\hbox{\tt\char`\ }} % visible space

\def\pt{\,{\rm pt}} % units of points, in math formulas
\def\em{\,{\rm em}} % units of ems, in math formulas
\def\<#1>{\leavevmode\hbox{$\langle$#1\/$\rangle$}} % syntactic quantity
\def\oct#1{\hbox{\rm\'{}\kern-.2em\it#1\/\kern.05em}} % octal constant
\def\hex#1{\hbox{\rm\H{}\tt#1}} % hexadecimal constant
\def\cstok#1{\leavevmode\thinspace\hbox{\vrule\vtop{\vbox{\hrule\kern1pt
        \hbox{\vphantom{\tt/}\thinspace{\tt#1}\thinspace}}
      \kern1pt\hrule}\vrule}\thinspace} % control sequence token

{\obeyspaces\gdef {\ }}
\def\parbreak{\hfil\break\indent\strut}
\def\stretch{\nobreak\hskip0pt plus2pt\relax}

% macros for non-centered displays
\outer\def\begindisplay{\obeylines\startdisplay}
{\obeylines\gdef\startdisplay#1
  {\catcode`\^^M=5$$#1\halign\bgroup\indent##\hfil&&\qquad##\hfil\cr}}
\outer\def\enddisplay{\crcr\egroup$$}

% (the following \begin...\end-type macros do not appear in Appendix E)
% macros for demonstrating math constructions
\outer\def\beginmathdemo{$$\advance\baselineskip by2pt
  \halign\bgroup\indent\hbox to 160pt{##\hfil}&$##$\hfil\cr\noalign{\vskip-2pt}}
\outer\def\begindisplaymathdemo {$$\advance\baselineskip by15pt
  \halign\bgroup\indent\hbox to 160pt{##\hfil}&$\displaystyle{##}$\hfil\cr
  \noalign{\vskip-15pt}}
\outer\def\beginlongmathdemo{$$\advance\baselineskip by2pt
  \halign\bgroup\indent\hbox to 210pt{##\hfil}&$##$\hfil\cr\noalign{\vskip-2pt}}
\outer\def\beginlongdisplaymathdemo {$$\advance\baselineskip by15pt
  \halign\bgroup\indent\hbox to 210pt{##\hfil}&$\displaystyle{##}$\hfil\cr
  \noalign{\vskip-15pt}}
\outer\def\endmathdemo{\egroup$$}

% macros for font tables
\def\oddline#1{\cr
  \noalign{\nointerlineskip}
  \multispan{19}\hrulefill&
  \setbox0=\hbox{\lower 2.3pt\hbox{\hex{#1x}}}\smash{\box0}\cr
  \noalign{\nointerlineskip}}
\def\evenline{\cr\noalign{\hrule}}
\def\chartstrut{\lower4.5pt\vbox to14pt{}}
\def\beginchart#1{$$\postdisplaypenalty=-10000 \global\count@=0 #1
  \halign to\hsize\bgroup
    \chartstrut##\tabskip0pt plus10pt&
    &\hfil##\hfil&\vrule##\cr
    \lower6.5pt\null
    &&&\oct0&&\oct1&&\oct2&&\oct3&&\oct4&&\oct5&&\oct6&&\oct7&\evenline}
\def\endchart{\raise11.5pt\null&&&\hex 8&&\hex 9&&\hex A&&\hex B&
  &\hex C&&\hex D&&\hex E&&\hex F&\cr\egroup$$}
\def\:{\setbox0=\hbox{\char\count@}%
  \ifdim\ht0>7.5pt\reposition
  \else\ifdim\dp0>2.5pt\reposition\fi\fi
  \box0\global\advance\count@ by1 }
\def\reposition{\setbox0=\hbox{$\vcenter{\kern2pt\box0\kern2pt}$}}
\def\normalchart{%
  &\oct{00x}&&\:&&\:&&\:&&\:&&\:&&\:&&\:&&\:&&\oddline0
  &\oct{01x}&&\:&&\:&&\:&&\:&&\:&&\:&&\:&&\:&\evenline
  &\oct{02x}&&\:&&\:&&\:&&\:&&\:&&\:&&\:&&\:&&\oddline1
  &\oct{03x}&&\:&&\:&&\:&&\:&&\:&&\:&&\:&&\:&\evenline
  &\oct{04x}&&\:&&\:&&\:&&\:&&\:&&\:&&\:&&\:&&\oddline2
  &\oct{05x}&&\:&&\:&&\:&&\:&&\:&&\:&&\:&&\:&\evenline
  &\oct{06x}&&\:&&\:&&\:&&\:&&\:&&\:&&\:&&\:&&\oddline3
  &\oct{07x}&&\:&&\:&&\:&&\:&&\:&&\:&&\:&&\:&\evenline
  &\oct{10x}&&\:&&\:&&\:&&\:&&\:&&\:&&\:&&\:&&\oddline4
  &\oct{11x}&&\:&&\:&&\:&&\:&&\:&&\:&&\:&&\:&\evenline
  &\oct{12x}&&\:&&\:&&\:&&\:&&\:&&\:&&\:&&\:&&\oddline5
  &\oct{13x}&&\:&&\:&&\:&&\:&&\:&&\:&&\:&&\:&\evenline
  &\oct{14x}&&\:&&\:&&\:&&\:&&\:&&\:&&\:&&\:&&\oddline6
  &\oct{15x}&&\:&&\:&&\:&&\:&&\:&&\:&&\:&&\:&\evenline
  &\oct{16x}&&\:&&\:&&\:&&\:&&\:&&\:&&\:&&\:&&\oddline7
  &\oct{17x}&&\:&&\:&&\:&&\:&&\:&&\:&&\:&&\:&\evenline}

% (now Appendix E resumes again)
% macros for verbatim scanning
\chardef\other=12
\def\ttverbatim{\begingroup
  \catcode`\\=\other
  \catcode`\{=\other
  \catcode`\}=\other
  \catcode`\$=\other
  \catcode`\&=\other
  \catcode`\#=\other
  \catcode`\%=\other
  \catcode`\~=\other
  \catcode`\_=\other
  \catcode`\^=\other
  \obeyspaces \obeylines \tt}

\outer\def\begintt{$$\let\par=\endgraf \ttverbatim \parskip=\z@
  \catcode`\|=0 \rightskip-5pc \ttfinish}
{\catcode`\|=0 |catcode`|\=\other % | is temporary escape character
  |obeylines % end of line is active
  |gdef|ttfinish#1^^M#2\endtt{#1|vbox{#2}|endgroup$$}}

\catcode`\|=\active
{\obeylines \gdef|{\ttverbatim \spaceskip\ttglue \let^^M=\  \let|=\endgroup}}

% macros for syntax rules (again, not in Appendix E)
\def\[#1]{\silenttrue\xref|#1|\thinspace{\tt#1}\thinspace} % keyword in syntax
\def\beginsyntax{\endgraf\nobreak\medskip
  \begingroup \catcode`<=13 \catcode`[=13
  \let\par=\endsyntaxline \obeylines}
\def\endsyntaxline{\futurelet\next\syntaxswitch}
\def\syntaxswitch{\ifx\next\<\let\next=\syntaxrule
  \else\ifx\next\endsyntax\let\next=\endgroup
  \else\let\next=\continuerule\fi\fi \next}
\def\continuerule{\hfil\break\indent\qquad}
\def\endsyntax{\medbreak\noindent}
{\catcode`<=13 \catcode`[=13
  \global\let<=\< \global\let[=\[
  \gdef\syntaxrule<#1>{\endgraf\indent\silentfalse\xref\<#1>}}
\def\is{\ $\longrightarrow$ }
\def\alt{\ $\vert$ }

% macros to demarcate lines quoted from TeX source files
\def\beginlines{\par\begingroup\nobreak\medskip\parindent\z@ \obeylines
  \hrule\kern1pt\nobreak \everypar{\strut}}
\def\endlines{\kern1pt\hrule\endgroup\medbreak\noindent}
\def\weakendlines{\kern1pt\hrule\endgroup\medskip\noindent}
\def\finalendlines{\kern1pt\hrule\endgroup\medbreak}

\outer\def\exercise{\medbreak
  \global\advance\exno by 1
  \noindent\llap{\manual\char'170\rm\kern.15em}% triangle in margin
  {\ninebf EXERCISE \bf\chapno.\the\exno}\par\nobreak\noindent}
\def\dexercise{\global\advance\exno by 1
  \llap{\manual\char'170\rm\kern.15em}% triangle in indented space
  {\eightbf EXERCISE \bf\chapno.\the\exno}\hfil\break}
\outer\def\dangerexercise{\d@nger \dexercise}
\outer\def\ddangerexercise{\dd@nger \dexercise}

\newwrite\ans
\immediate\openout\ans=answers % file for answers to exercises
\outer\def\answer{\par\medbreak
  \immediate\write\ans{}
  \immediate\write\ans{\string\ansno\chapno.\the\exno:}
  \copytoblankline}
\def\copytoblankline{\begingroup\setupcopy\copyans}
\def\setupcopy{\def\do##1{\catcode`##1=\other}\dospecials
  \catcode`\|=\other \obeylines}
{\obeylines \gdef\copyans#1
  {\def\next{#1}%
  \ifx\next\empty\let\next=\endgroup %
  \else\immediate\write\ans{\next} \let\next=\copyans\fi\next}}

% Editorial notes: some things to watch for.

% f |\ and f ^|\ => insert \/  [e.g., if\/ |\hbox|...]
% appendi => check for \null  [e.g., Appendix~B\null.]
% ly- => the hyphen is probably omittable
% ''. and '', => transpose to .'' and ,''
% dgement => dgment
% in MFbook: f@' and \MF, and \MF.

% Macros for drawing figures (not in Appendix E)
\def\hidehrule#1#2{\kern-#1\hrule height#1 depth#2 \kern-#2 }
\def\hidevrule#1#2{\kern-#1{\dimen0=#1
    \advance\dimen0 by#2\vrule width\dimen0}\kern-#2 }
% \makeblankbox puts rules at the edges of a blank box
% whose dimensions are those of \box0 (assuming nonnegative wd,ht,dp)
% #1 is rule thickness outside, #2 is rule thickness inside
\def\makeblankbox#1#2{\hbox{\lower\dp0\vbox{\hidehrule{#1}{#2}%
    \kern-#1% overlap the rules at the corners
    \hbox to\wd0{\hidevrule{#1}{#2}%
      \raise\ht0\vbox to #1{}% set the vrule height
      \lower\dp0\vtop to #1{}% set the vrule depth
      \hfil\hidevrule{#2}{#1}}%
    \kern-#1\hidehrule{#2}{#1}}}}
\def\maketypebox{\makeblankbox{0pt}{1pt}}
\def\makelightbox{\makeblankbox{.2pt}{.2pt}}

% \box\bigdot is a null box with a bullet at its reference point
\newbox\bigdot \newbox\smalldot
\setbox0=\hbox{$\vcenter{}$} % \ht0 is the axis height
\setbox1=\hbox to\z@{$\hss\bullet\hss$} % bullet is centered on the axis
\setbox\bigdot=\vbox to\z@{\kern-\ht1 \kern\ht0 \box1 \vss}
\setbox1=\hbox to\z@{$\hss\cdot\hss$} % cdot is centered on the axis
\setbox\smalldot=\vbox to\z@{\kern-\ht1 \kern\ht0 \box1 \vss}

% \arrows makes things like <--- text --->
\def\arrows#1#2{% #1=width, #2=text
  {\setbox0=\hbox{$\mkern-2mu\mathord-\mkern-2mu$}
    \hbox to #1{\kern-.055556em$\leftarrow\mkern-6mu$%
      \cleaders\copy0\hfil
      \kern.4em #2\kern.4em
      \cleaders\copy0\hfil
      $\mkern-6mu\rightarrow$\kern-.055556em}}}

% \samplebox makes the outline of a box, with big dot at reference point
\def\samplebox#1#2#3#4{% #1=ht, #2=dp, #3=wd, #4=text
  {\setbox0=\vtop{\vbox to #1{\hbox to #3{}\vss}
      \nointerlineskip
      \vbox to #2{}}% now \box0 has the desired ht, dp, and wd
    \hbox{\copy\bigdot
      \vrule height.2pt depth.2pt width#3%
      \kern-#3%
      \makelightbox
      \kern-#3%
      \raise#1\vbox{\hbox to #3{\hss#4\hss}
        \kern 3pt}}}}

% \sampleglue makes glue between sample boxes
\newdimen\varunit
\varunit=\hsize \advance\varunit by-2\parindent
\divide\varunit by 58 % illustrations in Chapter 12
\def\sampleglue#1#2{% #1=width, #2=text
  \vtop{\hbox to #1{\xleaders\hbox to .5\varunit{\hss\copy\smalldot\hss}\hfil}
    \kern3pt
    \tabskip \z@ plus 1fil
    \halign to #1{\hfil##\cr#2\cr}}}

% Indexing macros
\newif\ifproofmode
\proofmodetrue % this should be false when making camera-ready copy
\newwrite\inx
\immediate\openout\inx=index % file for index reminders
\newif\ifsilent
\def\specialhat{\ifmmode\def\next{^}\else\let\next=\beginxref\fi\next}
\def\beginxref{\futurelet\next\beginxrefswitch}
\def\beginxrefswitch{\ifx\next\specialhat\let\next=\silentxref
  \else\silentfalse\let\next=\xref\fi \next}
\catcode`\^=\active \let ^=\specialhat
\def\silentxref^{\silenttrue\xref}

\def\marginstyle{\vrule height6pt depth2pt width\z@ \sevenrm}

\chardef\bslash=`\\
\def\xref{\futurelet\next\xrefswitch}
\def\xrefswitch{\begingroup
  \ifx\next|\aftergroup\vxref % case 1 or 2, |arg| or |\arg|
  \else\ifx\next\<\aftergroup\anglexref % case 3, "\<arg>" means angle brackets
    \else\aftergroup\normalxref \fi\fi\endgroup} % case 0, "{arg}"
\def\vxref|{\catcode`\\=\active \futurelet\next\vxrefswitch}
\def\vxrefswitch#1|{\catcode`\\=0
  \ifx\next\empty\def\xreftype{2}%
    \def\next{{\tt\bslash\text}}% type 2, |\arg|
  \else\def\xreftype{1}\def\next{{\tt\text}}\fi % type 1, |arg|
  \edef\text{#1}\makexref}
{\catcode`\|=0 \catcode`\\=\active |gdef\{}}
\def\anglexref\<#1>{\def\xreftype{3}\def\text{#1}%
  \def\next{\<\text>}\makexref}
\def\normalxref#1{\def\xreftype{0}\def\text{#1}\let\next=\text\makexref}
\def\makexref{\ifproofmode\insert\margin{\hbox{\marginstyle\text}}%
   \xdef\writeit{\write\inx{\text\space!\xreftype\space
     \noexpand\number\pageno.}}\writeit
   \else\ifhmode\kern\z@\fi\fi
  \ifsilent\ignorespaces\else\next\fi}
% the \insert (which is done in proofmode only) suppresses hyphenation,
% so the \kern\z@ is put in to give the same effect in non-proofmode.

% Internal cross references that may change
\def\sesame{61} % page number for Sesame Street quote
\def\bmiexno{20} % exercise number for bold math italic
\def\punishexno{1} % exercise number for `punishment'
\def\fracexno{6} % exercise number for `\frac'
\def\vshippage{31} % error message from `\vship'
\def\storypage{24} % listing of story.tex
\def\metaT{4} % exercise number for T of METAFONT
\def\xwhat{2} % exercise number for x3:=whatever
\def\Xwhat{2} % exercise number for whatever itself

\def\checkequals#1#2{\ifnum#1=#2\else
  \errmessage{Redefine \string#1 to be \the#2}\fi}

% Things for The METAFONTbook only
\ifx\MFmanual\!\else\endinput\fi

\def\!{\kern-.03em\relax}

\def\frac#1/#2{\leavevmode\kern.1em
  \raise.5ex\hbox{\the\scriptfont0 #1}\kern-.1em
  /\kern-.15em\lower.25ex\hbox{\the\scriptfont0 #2}}

\outer\def\displayfig #1 (#2){$$\advance\abovedisplayskip by 3pt
  \leftline{\indent\figbox{#1}{3in}{#2}\vbox}$$}
\def\rightfig #1 (#2 x #3) ^#4 {% #2 wide and #3 deep, raised #4
  \strut\vadjust{\setbox0=\vbox to 0pt{\vss
      \hbox to\pagewidth{\hfil
        \raise #4\figbox{#1}{#2}{#3}\vtop \quad}}
    \dp0=0pt \box0}}
\def\figbox#1#2#3#4{#4to#3{ % makes a box #2 wide and #3 deep
    \ifproofmode\kern0pt\hrule\vfill
    \hsize=#2 \baselineskip 6pt \fiverm\noindent\raggedright
    (Figure #1 will be inserted here; too bad you can't see it now.)
    \endgraf\vfill\hrule
    \else\vfill\hbox to#2{}\fi}}

\def\endsyntax{\begingroup\let\par=\endgraf\medbreak\endgroup\noindent}

\let\BEGINCHAPTER=\beginchapter
\def\beginchapter{\titlelsl=1pt \BEGINCHAPTER}
\def\beginChapter{\titlelsl=2pt \BEGINCHAPTER}

\def\decreasehsize #1 {\advance\hsize-#1}
\def\restorehsize{\hsize=\pagewidth}

\catcode`\@=\active
\catcode`\"=\active
\def\ttverbatim{\begingroup \catcode`\@=\other \catcode`\"=\other
  \catcode`\\=\other
  \catcode`\{=\other
  \catcode`\}=\other
  \catcode`\$=\other
  \catcode`\&=\other
  \catcode`\#=\other
  \catcode`\%=\other
  \catcode`\~=\other
  \catcode`\_=\other
  \catcode`\^=\other
  \obeyspaces \obeylines \tt}
\def\setupcopy{\def\do##1{\catcode`##1=\other}\dospecials
  \catcode`\|=\other \catcode`\@=\other \catcode`\"=\other \obeylines}
\def\_{\leavevmode \kern.06em \vbox{\hrule width.3em}}
\def@#1@{\begingroup\def\_{\kern.04em
    \vbox{\hrule width.3em height .6pt}\kern.08em}%
  \ifmmode\mathop{\bf#1}\else\hbox{\bf#1\/}\fi\endgroup}
\def"#1"{\hbox{\it#1\/\kern.05em}} % italic type for identifiers
\def\xrefswitch{\begingroup
  \ifx\next|\aftergroup\vxref % case 1, |arg| or |\arg|
  \else\ifx\next@\aftergroup\boldxref % case 2, "@arg@" means boldface
  \else\ifx\next"\aftergroup\italxref % case 4, ""arg"" means boldface
  \else\ifx\next\<\aftergroup\anglexref % case 3, "\<arg>" means angle brackets
    \else\aftergroup\normalxref \fi\fi\fi\fi\endgroup} % case 0, "{arg}"
\def\boldxref@#1@{\def\xreftype{2}\def\text{#1}%
  \def\next{@\text@}\makexref}
\def\italxref"#1"{\def\xreftype{4}\def\text{#1}%
  \def\next{"\text"}\makexref}

\def\pyth+{\mathbin{++}}
\def\0{\raise.7ex\hbox{$\scriptstyle\#$}}
\def\to{\mathrel{\ldotp\ldotp}}
\def\dashto{\mathrel{\hbox{-\thinspace-\kern-.05em}}}
\def\ddashto{\mathrel{\hbox{-\thinspace-\thinspace-\kern-.05em}}}
\def\round{\mathop{\rm round}}
\def\angle{\mathop{\rm angle}}
\def\rmsqrt{\mathop{\rm sqrt}}
\def\reverse{\mathop{\rm reverse}}
\def\curl{\mathop{\rm curl}}
\def\tension{\mathop{\rm tension}}
\def\atleast{\mathop{\rm atleast}}
\def\controls{\mathop{\rm controls}}
\def\and{\,{\rm and}\,}
\def\cycle{{\rm cycle}}
\def\pickup{@pickup@ \thinspace}
\def\penpos#1{\hbox{\it penpos}_{#1}}
\def\pentaper#1{\hbox{\it pentaper}_{#1}}

\chardef\hexa=1  % first hex
\chardef\hexb=2 % top and bot adjusted
\chardef\hexc=3 % same, bold
\chardef\hexd=4 % same, confined to box
\chardef\hexe=5 % penstroked hex
\chardef\Aa=6 % stick-figure A, golden ratio
\def\sevenAs{\char7\char8\char9\char10\char11\char12\char13} % same, variants
\chardef\Az=14 % same, with crooked bar
\chardef\Ab=15 % \Aa with rectilinear elliptical pen
\chardef\Ac=16 % same, with the ellipse tilted
\chardef\beana=17 % kidney bean, default pen
\chardef\beanb=18 % same, twice as bold
\chardef\beanc=19 % same, rectilinear elliptical pen
\chardef\beand=20 % same, with the ellipse tilted
\chardef\niba=21 % 10x rectilinear ellipse
\chardef\nibb=22 % same, with the ellipse tilted
\chardef\nibc=23 % same, 90 degrees titled
\chardef\IOT=24 % Ionian T
\chardef\IOS=25 % Ionian S
\chardef\IOO=26 % Ionian O
\chardef\IOI=27 % Ionian I
\chardef\cubea=28 % possible cube
\chardef\cubeb=29 % impossible cube
\chardef\bicentennial=30 % star with overlapping strokes
\chardef\oneu=31 % 1/4 of uuuu ornament
\chardef\circa=32 % quartercircle
\chardef\circb=33 % filled quartercircle
\chardef\circc=34 % rotated quartercircle
\chardef\circd=35 % cone
\chardef\circe=36 % concentric circles
\chardef\circf=37 % concentric diamonds
\chardef\fouru=38 % uuuu ornament
\chardef\fourc=39 % same, rotated
\chardef\seventh='140 % 1/7, to go with cmssqi8

\newdimen\apspix
\apspix=31448sp % 8 APS pixels = 52413.64sp, and I'm taking 60% of this
% to crude approximation, there are about 2\apspix per pt
\newdimen\blankpix \newdimen\Blankpix
\setbox0=\hbox{\manual P} \blankpix=\wd0 % approximately 1pt blank pixel
\setbox0=\hbox{\manual R} \Blankpix=\wd0 % approximately 3pt blank pixel

\def\leftheadline{\hbox to \pagewidth{%
    \vbox to 10pt{}% strut to position the baseline
    \llap{\tenbf\folio\kern1pc}% folio to left of text
    \def\MF{{\manual 89:;<=>:}}% slanted 10pt
    \tenit\rhead\hfil% running head flush left
    }}
\def\rightheadline{\hbox to \pagewidth{%
    \vbox to 10pt{}% strut to position the baseline
    \def\MF{{\manual 89:;<=>:}}% slanted 10pt
    \hfil\tenit\rhead\/% running head flush right
    \rlap{\kern1pc\tenbf\folio}% folio to right of text
    }}
\def\ttok#1{\leavevmode\thinspace\hbox{\vrule\vtop{\vbox{\hrule\kern1pt
        \hbox{\vphantom{\tt(j}\thinspace{\tt#1}\thinspace}}
      \kern1pt\hrule}\vrule}\thinspace} % token

\newdimen\tinypix \setbox0=\hbox{\sixrm0} \tinypix=5pt
\newdimen\pixcorr \pixcorr=\tinypix \advance\pixcorr by-\wd0
\def\pixpat#1#2#3#4{\vcenter{\sixrm\baselineskip=\tinypix
  \hbox{#1\kern\pixcorr#2}\hbox{#3\kern\pixcorr#4}}}

\font\rand=random


==> postfigs.tex <==
%
%
%
%
%
\figitem{samp}{(A) shows the essential structure of the samples.
Electron transfer through the
tunnel barrier brings the electron gases in the substrate and the
quantum well in equilibrium. The density of electrons in the quantum
well may be varied through application of a gate bias ($V_{gate}$ in
the figure).
Capacitive coupling to the well allows us to measure both the
thermodynamic density of states (DOS) in the well and tunneling from
the well to the substrate.
(B)~displays the equivalent
model of the sample which is used in curve fitting to extract the
tunneling conductance and the density of states in the quantum well.}

\figitem{freq}{Capacitance and loss tangent of a 200 $\mu$m mesa
etched on sample {\bf B}. The solid and dotted curves are fits from
the circuit model presented in Fig.\ \fign{samp}B. At low frequencies,
electron transfer from the substrate to the well can take place, and
the capacitance $C_{low}$ is measured. At frequencies high compared to
the RC time of the tunnel barrier, no electron transfer to the well
takes place, and the measured capacitance, $C_{high}$
drops to a value consistent
with the distance from the top gate to the substrate layer.}

\figitem{nofield}{Capacitances $C_{low}$ (crosses) and $C_{high}$
(boxes), which are described in
the caption of Fig.\ \fign{freq},
determined from fits to capacitance vs.\ frequency data on
sample {\bf B}. The sharp increase in $C_{low}$ occurs as the well
begins to fill with electrons.
Here, there is no magnetic field applied and the temperature
is 4.2 K.}

\figitem{wfield}{Capacitances $C_{low}$ (crosses)
and $C_{high}$ (boxes) for sample {\bf
B} at 2.0 T and 1.9 K. Note the oscillations in the low frequency
capacitance. These arise from the Landau level density of states (DOS)
in the well. The
high frequency capacitance is insensitive to the DOS in the well and
does not display any such oscillations.}

\figitem{2.0TH}{Density of states ($\partial n/\partial\mu$)
vs.\ Fermi energy in sample {\bf B} at 2.0~T and 1.9~K
extracted using our model from the data presented the data of
Fig.\ \fign{wfield}. The vertical lines drawn are $\hbar\omega_c$
apart in energy. Note, one of the two unknown sample parameters in our
model was adjusted so as to keep two of the peaks $\hbar\omega_c$
apart. The fact that other peaks also fall $\hbar\omega_c$ apart is an
indication of the consistency of our model. The deviation of the
spacing between the first and second peaks arises from inhomogeneous
``puddling'' of electrons in the well as the well is emptied. The
first peak is thus outside of the region of validity of our model.}

\figitem{intlev}{The integrated ``lever-arm' used to convert DOS
results from gate bias to Fermi energy in the well. The lever-arm along
with the DOS is determined directly from the data. The flatter
regions of the curve occur where the DOS in the well is high, and
addition of electrons to the well changes the Fermi energy little. The
steeper regions occur where the DOS is low.}

%
%
%
%
%

%
%

\figitem{fold}{$\partial n/\partial\mu$ from the data of Fig.\ \fign{fit4ta}
(for our purposes here, assumed to be the same as the zero
temperature DOS) convolved with the
derivative of the Fermi Distribution function at 7.0~K (circles), compared to
$\partial n/\partial\mu$ determined from the data at 7.0~K (crosses). The
excellent agreement between the 7.0~K and the results of the
convolution serves as another consistency check of the model.
The slight deviation of the peaks is believed to arise largely from
the fact that the data used in the convolution is not the zero
temperature DOS but instead at 1.8~K.}

\figitem{fit4ta}{$\partial n/\partial\mu$ of sample {\bf A} at 4.0~T and
1.8~K. Circles are data.
The solid curve is a fit to Lorentzian lineshapes, and the dotted
curve is a fit to Gaussian shapes plus an added energy independent
background of $1.54\times10^{13}$eV$^{-1}$cm$^{-2}$.}

\figitem{fit3ta}{$\partial n/\partial\mu$ of sample {\bf A} at 3.0~T and
1.9~K. Circles are data.
The solid curve is a fit to Lorentzian lineshapes, and the dotted
curve is a fit to Gaussian shapes with a background. In this case, the
best fit is obtained with a negligibly small background. The
Lorentzians fit the underlying lineshape better than the Gaussians
and more successfully characterize the interlevel DOS.}

%
%
%

%
%
%
%

\figitem{widths}{Halfwidths, $\Gamma$ from Lorentzian fits,
of Landau levels in sample {\bf A}
plotted as a function of the
density at which the Landau level peak occurs for magnetic fields of
2, 3, and 4 Tesla. The solid line is a 2nd order polynomial fit to all
of the data and is meant as a guide to the eye. The figure suggests
that the Landau level widths are independent of magnetic field
strength.}

==> refmac.tex <==
% refmac.tex 11-10-87
%
% 11-10-87; remove extra spaces from \citedef
%
% 8-6-87; CHANGE \makelistmacro SO THAT SPACES BEFORE KEYWORDS IN
% CITATIONS ARE IGNORED.  Add \quietcite command to add a reference
% without printing the number.  (This is usefull for citations that
% initially appear in table or figure captions which appear AFTER the
% references in a draft.)  Also add additional jounal abbreviations. 
%
% 8-25-86; modifcation of refmac.tex 8-18 and 6-30-86: now keys may by
% separated by commas or by the original \\{key}, and numbers can be
% refered to in the text with the \refnumber{keys} command.
%
%
% This contains the TEX macros for citing keywords from a bibliography.
% (The bibliography must be appear in the document prior to listing the
% references.) To use these macros include:
%	\input ho>lloyd>refmac.tex
% in the beginning of the document file.
%
% To enter items in the bibliography, use the command:
%	\bibitem{keyword(s)}{bibliographic text}
%
% The items in the bibliography can appear in arbitrary order;
% to cite items in the bibliographic list, use the command:
%	\cite{key1,key2,...,keyn}
% or after a period:
%	\pcite{key1,key2,...,keyn}
% TEX will decide if the keyword has been cited previously and assign
% a reference number accordingly.  The numbers appear sequentially in
% the text (as superscripts), and if three or more sequencial reference
% numbers are cited, the sequence is hyphenatd, i.e. 3-6.  Note that
% the keywords can be cited in any order.  To cite an item without printing
% the number at that time, use the command:
%       \quietcite{key1,key2,...,keyn}
% This is usefull for citations that will appear in the draft AFTER the
% list of references, e.g. in a table or figure caption, so that an
% appropriate number can be assigned to the bibitem.
%
% The correct reference number(s) associated with a particular key(s)
% can be printed in the text (IN MATHMODE) by saying
%       \refnumber{key1,key2,...,keyn}
% eg. "In Ref. [\refnumber{key1}]" would result in "In Ref. [1]".
%
% The command
%	\listrefs	or	\listrefsAIP
% will list all the references in the order of citation.  The \listrefs
% will appear in the JVST format (ref numbers hanging).  The \listrefsAIP
% uses the AIP format (each reference a separate paragraph).
%
% If you wish to redefine the \listrefs format use:
%	\long\def\printref#1#2{newformat}
% where #1 is the reference number and #2 is the reference text.
%
% Also defined are commands for the abbreviations for commonly cited
% references, defined as:
%	\JOURNAL{volume no.}{page}{year}
% which will expand as: J.\ Abbrev.\ {\bf vol}, page (year)
% The following journals are defined:
%       \AP -> Appl. Phys.
%       \APL -> Appl. Phys. Lett.
%	\ASS -> Appl. Surf. Sci.
%       \CPL -> Chem. Phys. Lett.
%       \JACS -> J. Am. Chem. Soc.
%       \JAP -> J. Appl. Phys.
%	\JCAT -> J. Catal.
%	\JCP -> J. Chem. Phys.
%	\JESRP -> J. Electron Spectrosc. Relat. Phenom.
%       \JPC -> J. Phys. Chem.
%	\JVST -> J. Vac. Sci. Technol.
%       \JVSTA -> J. Vac. Sci. Technol. A
%       \JVSTB -> J. Vac. Sci. Technol. B
%       \LANG -> Langmuir
%       \PR -> Phys.Rev.
%	\PRB -> Phys. Rev. B	(will expand as Phys.\ Rev.\ B {\bf vol.} ...)
%	\PRL -> Phys. Rev. Lett.
%	\RSI -> Rev. Sci. Intsrum.
%	\SS -> Surf. Sci.
%       \SSC -> Solid State Commun.
%       \SSE -> Solid--State Electron.
%       \SSR -> Surf. Sci. Rep.
%	\VAC -> Vacuum
%
% Also defined is Ibach and Mills EELS book:
%       \IBACH -> H. Ibach and D. L. Mills, Electron Energy Loss Spectroscopy
%                 and Surface Vibrations (Academic, New York, 1982)
% see Lloyd Whitman with additional suggestions.
%
% The rest of the file are the macros:
%
%\tracingmacros=1%	debugging switches
%\tracingmacros=2
%\tracingcommands=1
%\tracingcommands=2
%\tracingonline=1
%
\message{** REFMAC.TEX ....reference numbering macros....LJW.11.10.87 **}
%
\def\cite#1{\buildlist{#1}\updaterefs{\listed}$^{\citerefs{\listed}}$}
\def\pcite#1{\cite{#1}\hskip 4.4443pt plus 4.99997pt minus 0.37036pt}
%
\def\refnumber#1{\buildlist{#1}\updaterefs{\listed}\citerefs{\listed}}
%
\def\quietcite#1{\buildlist{#1}\updaterefs{\listed}}
%
% The \buildlist and \makelistmacro macros create the listmacro if
% the keys are separated by commas, otherwise it defines
% the list macro to be the actual contents of the { }.  The \oldcheck
% macro checks if the delimiters are \\'s.
%
\newif\ifold
\def\buildlist#1{\oldcheck#1@%
                 \ifold\def\listed{#1}%
                 \else\def\listed{}\makelistmacro#1,@%
                 \fi}
\def\oldcheck#1#2@{\def\delim{#1}\def\olddelim{\\}%
                  \ifx\delim\olddelim%
                     \oldtrue\def\\{}%
                  \else %
                     \oldfalse %
                  \fi}
\def\makelistmacro#1#2,#3@{\add{#1#2}\to{\listed}%
                         \def\restoflist{#3}%
                         \ifx\restoflist\empty\relax%
                         \else\makelistmacro#3@%
                         \fi}
%
\def\refkeys{}%		the list of keywords; accumulated as cited
\def\biblist{}%		the list of keywords and text; built by \bibitem
%
\newcount\citenum%	the number of items in a given \cite command
\newif\ifmember
%
%
% The \updaterefs macro decides whether the cited keys have been
% cited previously by checking them against the \refkeys list.
% (For each cited key, it only checks the list until the key is found.)
% If a key has not been cited before, it is added to the \reflist list.
%
\def\updaterefs#1{\citenum=0%
                 \def\\##1{\updatedef{##1}}%
                 #1}%
%
\def\updatedef#1{\advance\citenum by 1%
                 \ifx\refkeys\empty%	For the first citation, start the list
                    \add{#1}\to{\refkeys}%
                 \else%
                    \memberfalse%
                    \ismember{#1}\of{\refkeys}%	check if key is on list
                    \def\\##1{\updatedef{##1}}% reset the \\ definition, which
                    \ifmember%			gets changed during \ismember
                    \else%
                       \add{#1}\to{\refkeys}%	If key isn't on list, add it
                    \fi%
                 \fi}%
%
%
% The \ismember#1\of#2 macro compares item #1 with each item on list #2,
% and sets \membertrue if it is on the list.
%
\def\ismember#1\of#2{\def\given{#1}%
                     \def\\##1{\def\next{##1}%
                               \ifmember%
                               \else%
                                  \ifx\next\given%
                                      \membertrue%
                                  \fi%
                               \fi}%
                     #2}%
%
%
% The \add#1\to#2 macro adds item #1 to list #2.
%
\toksdef\ta=0
\toksdef\tb=2
\long\def\add#1\to#2{\ta={\\{#1}}%
                     \tb=\expandafter{#2}%
                     \global\edef#2{\the\tb\the\ta}}%
%
%
%\def\cited{}% debugging list
\newcount\refnum% the reference number, as determined by the order of citation
\newcount\seqnum% the number in sequence
\newcount\seqfirst% the first in a sequence
\newcount\seqlast% the last in a sequence
%
%
% The \citerefs macro sequentially prints the reference numbers of the
% cited keys, with sequences hyphenated.  It does this by comparing each
% key in the \refkeys list with the cited keys, keeping track of the ref
% number. When it finds a refkey that was cited, it starts a sequence,
% assigning the refnum to seqfirst.  The seqnum is advanced until a refkey
% is found that has NOT been cited or else the last cited key is matched.
% If the `sequence' contains only one number, it is printed; if it contains
% two numbers, they are both printed; if three or more numbers have been cited
% sequentially, they are printed `first-last'.  The appropriate punctuation
% is determined by checking whether the refnum is the last in the current
% citation.
%
\def\citerefs#1{\refnum=0%
                \seqnum=0%
                \def\\##1{\citedef{#1}{##1}}%
                \refkeys%
                \def\\##1{}}
%
\def\citedef#1#2{\ifnum\citenum>0
                     \advance\refnum by 1%
                     \memberfalse%
                     \ismember{#2}\of{#1}%	was refkey cited?
                     \def\\##1{\citedef{#1}{##1}}%	redefine \\
                     \ifmember
                        \advance\citenum by-1 %
%                        \add{#2}\to{\cited}
                        \ifnum\seqnum=0 %
                           \ifnum\citenum=0 %
                              \number\refnum %
                           \else %
                              \advance\seqnum by 1 %
                              \seqfirst=\refnum %
                           \fi %
                        \else %
                           \advance\seqnum by 1 %
                           \ifnum\citenum=0 %
                              \ifnum\seqnum=2 %
                                 \number\seqfirst ,\number\refnum %
                              \else %
                                 \number\seqfirst \hbox{--}\number\refnum %
                              \fi %
                           \else %
                              \seqlast=\refnum %
                           \fi %
                        \fi %
                     \else %
                        \ifnum\seqnum>2 %
                           \number\seqfirst \hbox{--}\number\seqlast ,%
                        \else %
                           \ifnum\seqnum=2 %
                              \number\seqfirst ,\number\seqlast ,%
                           \fi %
                           \ifnum\seqnum=1 %
                              \number\seqfirst ,%
                           \fi%
                        \fi%
                        \seqnum=0 %
                     \fi %
                  \fi}
%
%
% The macros \listrefs and \listrefsAIP list the references in the order of
% citation in the format described by \printref#1#2 and \printrefAIP#1#2.
% This is accomplished by searching the \biblist keys until a match is
% found with the refkey. (The \biblist has the format:
% \\{key1}\\{test1}\\{key2}\\{text2}\\...)
%
\long\def\listrefs{\refnum=0%
                   \def\\##1{\advance\refnum by 1%
                             \writeref{\number\refnum}{##1}}%
                   \refkeys}
%
\long\def\listrefsAIP{\refnum=0%
                      \parindent=15.5pt
                      \def\\##1{\advance\refnum by 1%
                                \ifnum\refnum>8
                                   \parindent=11pt%
                                \fi
                                \writerefAIP{\number\refnum}{##1}}%
                      \refkeys%
                      \parindent=20pt}
%
% \writeref does the searching and printing
%
\long\def\writeref#1#2{\memberfalse%
                       \def\nextkey{#2}%
                       \long\def\\##1\\##2{\def\nextbibkey{##1}%
                                           \ifmember
                                           \else
                                              \ifx\nextkey\nextbibkey
                                                 \membertrue
                                                 \printref{#1}{##2}
                                              \fi
                                           \fi}%
                       \biblist%
                       \def\\##1{\advance\refnum by 1%
                                 \writeref{\number\refnum}{##1}}}
%
\long\def\writerefAIP#1#2{\memberfalse%
                          \def\nextkey{#2}%
                          \long\def\\##1\\##2{\def\nextbibkey{##1}%
                                              \ifmember
                                              \else
                                                 \ifx\nextkey\nextbibkey
                                                    \membertrue
                                                    \printrefAIP{#1}{##2}
                                                 \fi
                                              \fi}%
                          \biblist%
                          \def\\##1{\advance\refnum by 1%
                                   \ifnum\refnum>8
                                      \parindent=11pt%
                                   \fi
                                   \writerefAIP{\number\refnum}{##1}}}
%
% \printref defines the reference format
%
\long\def\printref#1#2{\par\hang\indent\llap{$^{#1}$}\ignorespaces #2.}
%
\long\def\printrefAIP#1#2{\par$^{#1}$#2.}
%
%
% \bibitem builds the \biblist as described above using the \add macro
%
\def\bibitem#1#2{\add{#1}\to{\biblist}%
                 \add{#2}\to{\biblist}}
%
%
%
% The following journals are defined:
%
\def\AP#1#2#3{Appl.\ Phys.\ {\bf #1}, #2 (#3)}
\def\APL#1#2#3{Appl.\ Phys.\ Lett.\ {\bf #1}, #2 (#3)}
\def\ASS#1#2#3{Appl.\ Surf.\ Sci.\ {\bf #1}, #2 (#3)}
\def\CPL#1#2#3{Chem.\ Phys.\ Lett.\ {\bf #1}, #2 (#3)}
\def\JACS#1#2#3{J.\ Am.\ Chem.\ Soc.\ {\bf #1}, #2 (#3)}
\def\JAP#1#2#3{J.\ Appl.\ Phys.\ {\bf #1}, #2 (#3)}
\def\JCAT#1#2#3{J.\ Catal.\ {\bf #1}, #2 (#3)}
\def\JCP#1#2#3{J.\ Chem.\ Phys.\ {\bf #1}, #2 (#3)}
\def\JESRP#1#2#3{J.\ Electron Spectrosc.\ Relat.\ Phenom.\ {\bf #1}, #2 (#3)}
\def\JPC#1#2#3{J.\ Phys.\ Chem.\ {\bf #1}, #2 (#3)}
\def\JVST#1#2#3{J.\ Vac.\ Sci.\ Technol.\ {\bf #1}, #2 (#3)}
\def\JVSTA#1#2#3{J.\ Vac.\ Sci.\ Technol.\ A {\bf #1}, #2 (#3)}
\def\JVSTB#1#2#3{J.\ Vac.\ Sci.\ Technol.\ B {\bf #1}, #2 (#3)}
\def\LANG#1#2#3{Langmuir {\bf #1}, #2 (#3)}
\def\PR#1#2#3{Phys.\ Rev.\ {\bf #1}, #2 (#3)}
\def\PRB#1#2#3{Phys.\ Rev.\ B {\bf #1}, #2 (#3)}
\def\PRL#1#2#3{Phys.\ Rev.\ Lett.\ {\bf #1}, #2 (#3)}
\def\RSI#1#2#3{Rev.\ Sci.\ Instrum.\ {\bf #1}, #2 (#3)}
\def\SS#1#2#3{Surf.\ Sci.\ {\bf #1}, #2 (#3)}
\def\SSC#1#2#3{Solid State Commun.\ {\bf #1}, #2 (#3)}
\def\SSE#1#2#3{Solid--State Electron.\ {\bf #1}, #2 (#3)}
\def\SSR#1#2#3{Surf.\ Sci.\ Rep.\ {\bf #1}, #2 (#3)}
\def\VAC#1#2#3{Vacuum {\bf #1}, #2 (#3)}
%
% In addition, Ibach and Mills is defined (with no concluding punctuation)
\def\IBACH{H.~Ibach and D.~L.~Mills, {\it Electron Energy Loss Spectroscopy
and Surface Vibrations} (Academic, New York, 1982)}
%

